Improving the Harmony of the Composite Image by Spatial-Separated Attention Module

Image composition is one of the most important applications in image processing. However, the inharmonious appearance between the spliced region and background degrade the quality of the image. Thus, we address the problem of Image Harmonization: Given a spliced image and the mask of the spliced region, we try to harmonize the "style" of the pasted region with the background (non-spliced region). Previous approaches have been focusing on learning directly by the neural network. In this work, we start from an empirical observation: the differences can only be found in the spliced region between the spliced image and the harmonized result while they share the same semantic information and the appearance in the non-spliced region. Thus, in order to learn the feature map in the masked region and the others individually, we propose a novel attention module named Spatial-Separated Attention Module (S2AM). Furthermore, we design a novel image harmonization framework by inserting the S2AM in the coarser low-level features of the Unet structure in two different ways. Besides image harmonization, we make a big step for harmonizing the composite image without the specific mask under previous observation. The experiments show that the proposed S2AM performs better than other state-of-the-art attention modules in our task. Moreover, we demonstrate the advantages of our model against other state-of-the-art image harmonization methods via criteria from multiple points of view. Code is available at https://github.com/vinthony/s2am

==> IEEEbibo.tex <==

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip]{figures/xiaodong_cun.jpg}}]{Xiaodong Cun}
is currently a Ph.D student at the University of Macau. Before that, he received his B.Sc and M.Sc. degrees in Computer Science from Xidian University and University of Macau in 2015 and 2018 respectively. He is focusing on the application of the deep learning-based methods for Image Processing and Computational Photography.
\end{IEEEbiography}

% if you will not have a photo at all:
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip]{figures/chiman_pun.jpg}}]{Chi-Man Pun}
~(M’09-SM’10) received his B.Sc. and M.Sc. degrees in Software Engineering from the University of Macau in 1995 and 1998 respectively, and Ph.D. degree in Computer Science and Engineering from the Chinese University of Hong Kong in 2002. He was the Head of the Department of Computer and Information Science from 2014 to 2019, and is currently an Associate Professor at the Faculty of Science and Technology of the University of Macau. He has authored/co-authored more than 150 refereed scientific papers in international journals and conference proceedings. Dr. Pun has served as the General Chair for the 10th\&11th International Conference Computer Graphics, Imaging and Visualization~(CGIV2013, CGIV2014), and program/session chair for several other international conferences. He has also served as the editorial member/referee for many international journals such as IEEE Transactions on Pattern Analysis and Machine Intelligence, IEEE Transactions on Information Forensics and Security, IEEE Transactions on Image Processing, Pattern Recognition, etc. His research interests include Information Security, Forensic and Privacy for Multimedia; Image Processing and Pattern Recognition.
\end{IEEEbiography}


